Point Intervention: Improving ACVP Test Vector Generation Through Human Assisted Fuzzing

Automated Cryptographic Validation Protocol (ACVP) is an existing protocol that is used to validate a software or hardware cryptographic module automatically. In this work, we present a system providing the method and tools to produce well-covering tests in ACVP format for cryptographic libraries. The system achieves better coverage than existing fuzzing methods by using a hybrid approach to fuzzing cryptographic primitives. In addition, the system offers a framework that allows to creates easily and securely create testing modules for cryptographic libraries. The work demonstrates how this system has been used to improve automated testing of NSS (Network Security Services), a popular cryptographic library, detect its vulnerabilities and suggest ways to improve and further develop the ACVP test format.

==> Makefile <==
SHELL := /bin/bash

FILE=manuscript
BIBALIAS=alias.bib
LOG_SEP="*******************************************************************************"
DIR_ARXIV=arxiv
TEXSRC:=$(wildcard *.tex)
IACRTRANS := $(shell grep '^\\IACRTRANStrue' $(FILE).tex)

BIBMASTER ?= master.bib

TEXFOT        := $(shell command -v texfot 2> /dev/null)
LATEX         := $(TEXFOT) pdflatex -shell-escape
CHKTEX        := $(shell command -v chktex 2> /dev/null)
# ChkTeX manual: https://www.nongnu.org/chktex/ChkTeX.pdf
#
# Default chktex warnings are: `-wall -n19 -n21 -n22 -n30 -n41`
# We elevate them to full errors and enable also
#
# -e19: "You should use ASCII 39 for quote"
# -e41: "You ought to not use primitive TeX in LaTeX code"
#
# For completeness, here is a summary of the warnings that we keep
# disabled as in the default chktex configuration:
#
# -n21: "This command might not be intended"
# -n22: "Comment displayed"
# -n30: "Multiple spaces detected in output"
#
# Finally, we disable:
#
# -n2: "Non-breaking space should have been used"
# -n7: "Accents for i and j (\i, \j)"
# -n8: "Wrong length of dash may have been used"
# -n9: "Brackets/environments order mismatch"
# -n13: interspace
# -n44: vrulers are bad
CHKTEX_OPTS   := -eall -n21 -n22 -n30 \
                 -n2 -n7 -n8 -n9 -n13 -n44
LATEXPAND     := $(shell command -v latexpand 2> /dev/null)
LATEXPAND_OPT := --empty-comments --show-graphics
BIBTEX        := $(shell command -v bibtex 2> /dev/null)

## maybe this helps macos ppl
ifeq ($(origin GREP), undefined)
  ifneq (, $(shell which ggrep))
    GREP      := $(shell command -v ggrep 2> /dev/null)
  else
    GREP      := $(shell command -v grep 2> /dev/null)
  endif
endif
GREP_OPTS     := --line-number --color=always


all: test img $(FILE).pdf

img:
	@echo $(LOG_SEP)
	$(MAKE) -C $@

BIBTOOL       := $(shell command -v bibtool 2> /dev/null)
BIBTOOL_OPT   := --preserve.keys=on --preserve.key.case=on --print.align.key=0 --print.line.length=999 --print.use.tab=0 --apply.alias=on -q
$(FILE)_ro.bib: $(FILE).aux
	@echo $(LOG_SEP)
ifneq (,$(wildcard $(BIBMASTER)))
  ifeq (, $(shell which $(BIBTOOL)))
    $(error "No bibtool in $(PATH), try sudo apt install bibtool")
  endif
	@echo "INFO: $(BIBMASTER) exists."
	$(eval TMPAUX := $(shell mktemp --tmpdir=. --suffix=.aux))
	sed 's/^\\bibdata{/\\bibdataold{/g' $< > $(TMPAUX)
	@echo "@COMMENT{==== NB NB NB NB ====}" > $@
	@echo "@COMMENT{==== THIS FILE IS AUTO GENERATED}" >> $@
	@echo "@COMMENT{==== ANY CHANGES YOU MAKE WILL LIKELY BE LOST}" >> $@
	@echo "@COMMENT{==== DO NOT PUT MANUAL ENTRIES HERE}" >> $@
	@echo "@COMMENT{==== PUT THEM IN THE *_rw.bib FILE INSTEAD}" >> $@
	@echo "@COMMENT{==== NB NB NB NB ====}" >> $@
	$(BIBTOOL) $(BIBTOOL_OPT) -x $(TMPAUX) -i $(BIBMASTER) $(BIBALIAS) >> $@
	@rm -f $(TMPAUX)
	## NB: (BBB) Shameless bib hacking. Break glass in case of emergency.
	##@sed -i 's/^  doi   /  ALTdoi/' $@
	##@sed -i 's/^  isbn   /  ALTisbn/' $@
	##@sed -i 's/^  url   /  ALTurl/' $@
	##@sed -i 's/Lecture Notes in Computer Science/LNCS/' $@
	##@sed -i 's/^  editor   /  ALTeditor/' $@
	##@sed -i 's/^  booktitle   /  ALTbooktitle/' $@
	##@sed -i 's/^  altbooktitle/  booktitle   /' $@
else
	@echo "INFO: $(BIBMASTER) does not exist."
endif

$(FILE).aux: $(TEXSRC) img
	@echo $(LOG_SEP)
	$(LATEX) $(FILE)

$(FILE).pdf: $(TEXSRC) $(FILE)_rw.bib $(FILE)_ro.bib
	@echo $(LOG_SEP)
	$(BIBTEX) $(FILE)
	@echo $(LOG_SEP)
	$(LATEX) $(FILE)
	@echo $(LOG_SEP)
	$(LATEX) $(FILE)
	@while grep -q '^LaTeX Warning: Label(s) may have changed' $(FILE).log; do \
		echo $(LOG_SEP); \
		$(LATEX) $(FILE); \
	done

arxiv.tar.gz: $(FILE).pdf
	@echo $(LOG_SEP)
	@rm -fr $(DIR_ARXIV)
	@mkdir -p $(DIR_ARXIV)/img
	##sed -n 's|^File: \(img/.*pdf\) Graphic file (type pdf)|\1 $(DIR_ARXIV)/\1|p' $(FILE).log | xargs -n2 cp
	@cp -L Makefile.arxiv $(DIR_ARXIV)/Makefile
ifeq ($(IACRTRANS), )
	## normal: expand bib directly in tex
	##$(LATEXPAND) $(LATEXPAND_OPT) --output=$(DIR_ARXIV)/$(FILE).tex --expand-bbl=$(FILE).bbl $(FILE).tex 2>&1 | xargs -L1 -n1 cp --target-directory=$(DIR_ARXIV)/img
	## NB this loop instead of xargs is for compatability with non coreutils cp
	for f in $$($(LATEXPAND) $(LATEXPAND_OPT) --output=$(DIR_ARXIV)/$(FILE).tex --expand-bbl=$(FILE).bbl $(FILE).tex 2>&1 | grep -v "^Warning"); do cp -L $$f $(DIR_ARXIV)/img/; done
else
	## IACRTRANS: biblatex so no expanding, give bib files directly
	@cp -L $(FILE)_ro.bib $(DIR_ARXIV)/
	@cp -L $(FILE)_rw.bib $(DIR_ARXIV)/
	##$(LATEXPAND) $(LATEXPAND_OPT) --output=$(DIR_ARXIV)/$(FILE).tex $(FILE).tex 2>&1 | xargs -L1 -n1 cp --target-directory=$(DIR_ARXIV)/img
	## NB this loop instead of xargs is for compatability with non coreutils cp
	for f in $$($(LATEXPAND) $(LATEXPAND_OPT) --output=$(DIR_ARXIV)/$(FILE).tex $(FILE).tex 2>&1 | grep -v "^Warning"); do cp -L $$f $(DIR_ARXIV)/img/; done
endif
	## NB this "backup then remove" is for compatability with non coreutils sed
	sed -i'.tmp' 's/^\\ifLINUXBUILD/\\iftrue/g' $(DIR_ARXIV)/$(FILE).tex
	@rm -f $(DIR_ARXIV)/$(FILE).tex.tmp
	$(MAKE) -C $(DIR_ARXIV)
	@echo $(LOG_SEP)
	tar --exclude='build' --exclude='_minted-manuscript' -zcvf $@ -C $(DIR_ARXIV) .

arxiv.zip: arxiv.tar.gz
	@echo $(LOG_SEP)
	@rm -fr $(DIR_ARXIV)
	@mkdir -p $(DIR_ARXIV)
	tar -zxvf $< -C $(DIR_ARXIV)
	(cd $(DIR_ARXIV) && zip -rv ../$@ *)

anon:
	@touch $(FILE).tex .tmp.anon.tmp
	$(MAKE) $(FILE).pdf
	@rm .tmp.anon.tmp
	@touch $(FILE).tex

deepclean: clean
	$(MAKE) -C img clean

chktex:
	@printf "\n===== Running ChkTeX on $(FILE).tex =====\n"
	@printf "### See https://www.nongnu.org/chktex/ChkTeX.pdf\n\n\n"
	$(CHKTEX) $(CHKTEX_OPTS) $(FILE).tex
.PHONY: chktex

custom_tests: $(FILE).pdf
	@if $(GREP) $(GREP_OPTS) '\\ref{' $(TEXSRC); then \
		printf "\n===== replace ref with autoref =====\n"; \
		exit 1; \
	fi
	@if $(GREP) $(GREP_OPTS) '^\\paragraph' $(TEXSRC); then \
		printf "\n===== replace paragraph command with the Paragraph macro =====\n"; \
		exit 1; \
	fi
	@if $(GREP) $(GREP_OPTS) -P '\t' $(TEXSRC); then \
		printf "\n===== replace tabs with spaces =====\n"; \
		exit 1; \
	fi
	@if $(GREP) $(GREP_OPTS) '[[:blank:]]$$' $(TEXSRC); then \
		printf "\n===== remove trailing whitespace =====\n"; \
		exit 1; \
	fi
	@if $(GREP) $(GREP_OPTS) -P '^([^%]|\\%)*?[^\x00-\x7F]' $(TEXSRC); then \
		printf "\n===== non ASCII character detected: possible typesetting / render issue =====\n"; \
		exit 1; \
	fi
	@if $(GREP) $(GREP_OPTS) -E '\\(bf|it|tt|rm|sf|sl|em|sc)\>' $(TEXSRC); then \
		printf "\n===== deprecated modal command detected. See https://texfaq.org/FAQ-2letterfontcmd =====\n"; \
		exit 1; \
	fi
	@if $(GREP) $(GREP_OPTS) -E '\$$\$$' $(TEXSRC); then \
		printf "===== math formula spacing issue: $$$$ detected. See 1.6 at https://www.texlive.info/CTAN/info/l2tabu/english/l2tabuen.pdf =====\n"; \
		exit 1; \
	fi
	@if $(GREP) $(GREP_OPTS) 'There were undefined citations' $(FILE).log; then \
		printf "\n===== fix undefined citations =====\n"; \
		exit 1; \
	fi
	@if $(GREP) $(GREP_OPTS) 'Citation.*on page.*undefined.*' $(FILE).log; then \
		printf "\n===== fix undefined citations =====\n"; \
		exit 1; \
	fi
	@if $(GREP) $(GREP_OPTS) 'There were undefined references' $(FILE).log; then \
		printf "\n===== fix undefined references =====\n"; \
		exit 1; \
	fi
	@if $(GREP) $(GREP_OPTS) 'Warning.*multiply.*defined' $(FILE).log; then \
		printf "\n===== fix duplicate labels =====\n"; \
		exit 1; \
	fi
.PHONY: custom_tests

test: chktex custom_tests

clean:
	rm -fr $(DIR_ARXIV)
	rm -f $(FILE).{aux,bbl,blg,log,out,pdf} anon.tex tmp.*.aux arxiv.tar.gz arxiv.zip *-blx.bib *.run.xml *~

.PHONY: test img all clean deepclean anon



### Check common prerequisites for most targets
#
# These are expanded when the Makefile is first parsed, before selecting targets

ifeq (, $(shell which $(TEXFOT)))
  $(error "No texfot in $(PATH), try sudo apt install texlive-extra-utils")
endif

ifeq (, $(shell which $(CHKTEX)))
  $(error "No chktex in $(PATH), get it from TeXLive")
endif

ifeq (, $(shell which $(LATEXPAND)))
  $(error "No latexpand in $(PATH), try sudo apt install texlive-extra-utils")
endif

ifeq (, $(shell which $(BIBTEX)))
  $(error "No bibtex in $(PATH), try sudo apt install texlive-binaries")
endif

ifeq (, $(shell which $(GREP)))
  $(error "No ggrep or grep in $(PATH), try sudo apt install grep")
endif


==> background.tex <==
\section{Background}\label{sec:background}

\subsection{Automated Testing}

Computer software must be tested to verify its proper functioning. Many implementation issues exist because of human errors made by programmers, like not ensuring a program is checking all its
inputs for size to avoid attempts to access beyond the end of an array. Modern programming languages offer various mechanisms to avoid that, like advanced type systems. However, in writing
cryptographic software, performance is crucial, and such programs have to use direct access to memory, and, thus, they are usually written in languages like C or C++~\cite{rustytypes}. One of the
approaches to ensure low-level code is working as intended is external automated testing. Automated testing is a process to verify the execution of a program without human interaction,
which vastly reduces costs.
Usually testing features challenges issued to the program and validation of the answers, such as ``encrypting bytes A with key $\mathsf{K}$ should result in bytes B''. Tests can
be generated on demand or they can be pre-generated, and they either verify the results using a pre-existing value or an another program, or just verify the program execution went well. One important characteristic
of tests is coverage, the measure of how well the code is ``covered'' by tests, to ensure no code is untested.

\subsection{Fuzzing}

Often, well-covering test sets are produced by fuzz testing, or fuzzing for short. Fuzzing is a form of automatic testing which repeatedly runs the target software with mutated input. In recent years,
coverage-based grey-box fuzzing (CGF) has proven to be very effective in finding security issues~\cite{weizz}. CGF fuzzer instruments the code, inserting special markers which are used to gather the coverage data, and uses changes in coverage as a guide to
which areas of the input should be changed to maximize the coverage, thus effectively gaining some idea about structure of the input. However, it might take a lot of resources for a fuzzer to
randomly satisfy complicated criteria often needed to improve coverage. To reduce the costs, numerous additional approaches are being tried, like using hardware support~\cite{hwfuzz} and symbolic
execution~\cite{symfuzz}.

\subsection{ACVP}

Automated Cryptographic Validation Protocol ({ACVP})~\cite{acvp} is a protocol to automatically test software or hardware cryptographic modules~\cite{acvp-spec}. {ACVP} is developed by NIST\null. {ACVP}
includes a portable, human
understandable, universal format of test data based on JSON\null~\cite{json}.
The challenges and answers are usually transmitted by network from
an {ACVP} server to clients who wish to validate a library. ACVP supports many primitives by the way of
``subspecifications'', which describe a family of cryptographic primitives like ``Secure Hash''~\cite{acvp-sha}.

On July 17, 1995, the Cryptographic Algorithm Validation Program (CAVP) and the Cryptographic Module Validation Program (CMVP) were established by NIST to validate cryptographic modules~\cite{acvt}.
Originally, all CMVP communications and operations on submitted cryptographic modules happened only within testing laboratories. However, as technology advanced, industry demanded faster testing
cycles than that scheme could provide, the required human involvement resulted in mistakes, and modules could not be monitored after initial validation. To reduce the costs and time of validation while still
providing a high level of assurance, the Automated Cryptographic Validation Testing (ACVT) project has been started.

As part of ACVT project, NIST has designed and developed a protocol and software for automated algorithm testing. NIST has published specifications of the protocol~\cite{acvp}, source code for the
server~\cite{acvp-server}, and runs both demo and production servers for remote verification.

{ACVP} tests do not have a shared defined structure, but, as a rule, subspecifications describe similar layouts. Tests are distributed in form of ``vector sets''. Vector sets contain some shared
information like the algorithm and the subspecification revision, and an array of ``test groups''. Test groups, similarly, include shared information specific to the subspecification, and an array of
``tests''. Tests include the rest of the information. The cryptographic module being tested has to respond to a test vector set with ``test vector response'', which is structured in a similar way.
An example of an ACVP vector set can be seen in \autoref{listing:acvp-example}.

\begin{figure}[!ht]
\inputminted{json}{code/acvp.json}
\caption{Example of an ACVP test vector set, obtained from ACVP demo server}%
\label{listing:acvp-example}
\end{figure}

Multiple tools to work with ACVP exist, including \code{acvpproxy}~\cite{acvpproxy} that interacts with an ACVP server.
There is \code{acvpparser}~\cite{acvpparser} that works with cryptographic libraries to
run vector sets, and \code{libacvp}~\cite{libacvp} that does both. These tools are written in C and are rather low-level and hard to extend. As we need to work with ACVP tests in a specific way and
need to interact with other tools that examine the program execution, we chose to implement own library in \textbf{Rust}, a strongly-typed secure by design language.

